The role of plasma beta in global coronal models: Bringing balance back to the force

COCONUT is a global coronal magnetohydrodynamic model recently developed. In order to achieve robustness and fast convergence to steady-state, several assumptions have been made during its development, such as prescribing filtered photospheric magnetic maps for representing the magnetic field in the lower corona. This filtering leads to smoothing and lower magnetic field values at the inner boundary, resulting in an unrealistically high plasma beta.In this paper, we examine the effects of prescribing such filtered magnetograms and formulate a method for achieving more realistic plasma beta values without losing computational performance. We demonstrate the effects of the highly pre-processed magnetic maps and the resulting high plasma beta on the features in the domain. Then, in our new approach, we shift the inner boundary to 2 Rs and preserve the prescribed highly filtered magnetic map. This effectively reduces the prescribed plasma beta and leads to a more realistic setup. The method is applied on a magnetic dipole, a minimum (2008) and a maximum (2012) solar activity case, to demonstrate its effects. The results obtained with the proposed approach show significant improvements in the resolved density and radial velocity profiles, and far more realistic values of the plasma \{beta} at the boundary and inside the computational domain. This is also demonstrated via synthetic white light imaging and with the validation against tomography. The computational performance comparison shows similar convergence to a limit residual on the same grid when compared to the original setup. Considering that the grid can be further coarsened with this new setup, the operational performance can be additionally increased if needed. The newly developed method is thus deemed as a good potential replacement of the original setup for operational purposes.

==> referee_comments.tex <==
• Section 2.1: for some modelers it may be confusing why no heating, radiative cooling nor conductive heat flux terms are integrated in the model equations. The spatial extent of the model (1.01-25Rs) is stated in the section just after. But maybe just one, explicit sentence would be helpful to lift this ambiguity right away, explaining that the model starts from the low corona where those physical effects can be fairly neglected within an operational context.
• Caption Figure 1, “, with lmax if 30 (middle) and 15 (bottom)”: looks like a typo.
• Section 3.2, “If we investigate the plasma beta in Figure from Garry (2001), ”: another typo, which figure?
• Section 3.2, same sentence as above “...in the range of 0.3 to around 15.”: omission of the unit.
• Section 3.2: equations 7 and 8 should be placed before the definition of sin(Omega)=Rs/r and r^2=s^2+rho^2.
• Section 3.2: the meaning of the quantities “s” and “rho” has not been explained. I suppose “s” is the distance along the LOS. The acronym LOS for line-of-sight should be defined also, e.g. “…in order to compute, for each point, the polarized brightness integrated along the line-of-sight (LOS): ”.
• Section 3.3, “by a 1 Rs”: should be rephrased as “by one solar radius” to ease the reading.
• Section 3.3: Until this paragraph it remains quite disturbing that a “surface” magnetic map can be readily applied at 2Rs just by filtering small-scales and then adjusting the magnitude of the field. The implications on the assumed field topology should be discussed much earlier, at the very beginning in the introductory paragraphs of Section 3. Or at least, to be briefly mentioned there with reference to further discussion in section 3.3.
• Section 3.3, “the general position of the apex of the loop is still sufficiently accurate to create density enhancements in the right places, places, and –what matters for space weather forecasting are the conditions at 0.1 AU, not at 2 Rs, thus the effect of the inaccuracies close to the surface is diminished.”:
If the location is indeed more or less respected, the width of such structures is likely to be much larger compared to a BC applied at 1.01Rs. Which should result in wider streamer (and pseudo-streamer) flows and hence impacts the forecasting performances at 1 AU as well. A brief discussion on that potential impact would be welcome.
• Figures 9 and 12: As for the case with tomography, it would be beneficial to have an observation-based product to compare with the simulations. E.g. a coronagraph view of the observed white-light corona.
• Figures 9 and 12: In all other figures the horizontal and vertical coordinate axes have been omitted, which is ok since the comparisons are only qualitative here. But then these axes should be removed here as well (or inversely be added to all other figures with appropriate unit).

